An Order-Aware Dataflow Model for Parallel Unix Pipelines

We present a dataflow model for modelling parallel Unix shell pipelines. To accurately capture the semantics of complex Unix pipelines, the dataflow model is order-aware, i.e., the order in which a node in the dataflow graph consumes inputs from different edges plays a central role in the semantics of the computation and therefore in the resulting parallelization. We use this model to capture the semantics of transformations that exploit data parallelism available in Unix shell computations and prove their correctness. We additionally formalize the translations from the Unix shell to the dataflow model and from the dataflow model back to a parallel shell script. We implement our model and transformations as the compiler and optimization passes of a system parallelizing shell pipelines, and use it to evaluate the speedup achieved on 47 pipelines.

==> coarse-microbenchmarks-table.tex <==
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} l}
\toprule
Name ~&~ Script \\
\midrule
nfa-regex ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | tr A-Z a-z | grep '\(.\).*\1\(.\).*\2\(.\).*\3\(.\).*\4'! \\
sort ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | tr A-Z a-z | sort! \\
top-n ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | tr -cs A-Za-z '\n' | tr A-Z a-z | sort | uniq -c | sort -rn | sed ${N}q! \\
wf ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | tr -cs A-Za-z'\n' | tr A-Z a-z | sort | uniq -c | sort -rn | sed ${1}q! \\
spell ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | col -bx |tr -cs A-Za-z '\n' | tr A-Z a-z |tr -d '[:punct:]' |sort |uniq |!\\ ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!    comm -23 - $dict! \\
difference ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | sort | tr [:lower:] [:upper:] > s1 & cat $IN | sort |!\\ ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!    tr [:upper:] [:lower:] > s2 & diff -B s1 s2! \\
bi-grams ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | tr -cs A-Za-z '\n' | tr A-Z a-z | bigrams_aux | sort | uniq! \\
set-difference ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | cut -d ' ' -f 1 | sort > s1 & cat $IN | cut -d ' ' -f 1 | sort > s2 &!\\ ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!    comm -23 s1 s2! \\
shortest-scripts ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!cat $IN | xargs file | grep "shell script" | cut -d: -f1 | xargs -L 1 wc -l |!\\ ~&~ \lstinline[columns=fixed,basicstyle=\footnotesize\ttfamily]!    grep -v '^0$' | sort -n | head -15! \\
\bottomrule
\end{tabular*}

==> proof.tex <==
\begin{theorem}
    \label{thm:equi_exp}
    The following statements are true:
\[
    \begin{array}{rcl}
        e &\equiv& \relay(e)\\
        \concat(\splitc(e)) &\equiv& e\\
        &\#& \text{assuming }e\text{ computes to a packed set.}\\
        \splitc(\concat(e)) &\equiv& e\\
        &\#& \text{assuming }e\text{ computes to an unpacked set.}\\
        \concat(\concat(e)) &\equiv& \concat(e)\\
        \splitc(\splitc(e)) &\equiv& \splitc(e)\\
        \concat( \mathsf{map}^{f}_i(e_{j_1}, e_{j_2}, \ldots
        \splitc(e_{j_i}), \ldots e_{j_k})
        ) &\equiv&  f(e_{j_1}, e_{j_2},\ldots e_{j_i} \ldots, e_{j_k})
\\
        &\#&
        \text{Assuming }f\text{ is stateless with respect to index }i\\
         f(e_{j_1}, e_{j_2}, \ldots, e_{j_i} \ldots, e_{j_k}) &\equiv&  
         agg(e_{j_1}, e_{j_2}, \ldots,  
         m(e_{j_1}, e_{j_2}, \ldots, e_{j_k}) \ldots, e_{j_k}) \\
         &\#& \text{Where }m\text{ is the map function and } \\
         &\#& agg\text{ is
         the reduce function,} 
         \text{assuming }f\text{ is }\\ &\#& \text{Parallelizable Pure with respect to
         index }i 
    \end{array}
\]
\end{theorem}
\begin{proof}
    \begin{itemize}
        \item $\llbracket e \rrbracket_e = \llbracket \relay(e) \rrbracket_e$ as
            $\relay$ behaves as an identity function.
        \item Assuming $e$ computes to a packed set. $\llbracket e \rrbracket_e =
            [D^*]$. $\llbracket \splitc(e) \rrbracket_e = D^*$. 
            $\llbracket \concat(\splitc(e)) \rrbracket_e = [D^*] =
            \llbracket e \rrbracket_e$.
        \item Assuming $e$ computes to an unpacked set. $\llbracket e
            \rrbracket_e =
            D^*$. $\llbracket \concat(e) \rrbracket_e = [D^*]$. 
            $\llbracket \splitc(\concat(e)) \rrbracket_e = D^* =
            \llbracket e \rrbracket_e$.
        \item $\llbracket \concat(e) \rrbracket_e = [D^*] = \llbracket
            \concat(\concat(e)) \rrbracket_e$.
        \item $\llbracket \splitc(e) \rrbracket_e = [D^*] = \llbracket
            \splitc(\splitc(e)) \rrbracket_e$.
        \item $\llbracket f(e_1, \ldots e_i, \ldots e_m) \rrbracket_e = \llbracket
            f(\rrbracket e_1 \rrbracket_e, \rrbracket e_2 \rrbracket_e, \ldots,
            \rrbracket e_i \rrbracket_e, \ldots \rrbracket e_m
            \rrbracket_e)\rrbracket$
            which is equal to 
            \[\llbracket \concat(\mathsf{map}(\lambda.x~
            f(\rrbracket e_1 \rrbracket_e, \rrbracket e_2 \rrbracket_e, \ldots,
            \rrbracket x \rrbracket_e, \ldots \rrbracket e_m \rrbracket_e), 
            \llbracket \splitc(e_i) \rrbracket )\rrbracket\]
            by definition of Stateless commands.
        \item $\llbracket f(e_1, \ldots e_i, \ldots e_m) \rrbracket_e = \llbracket
            f(\llbracket e_1 \rrbracket_e, \llbracket e_2 \rrbracket_e, \ldots,
            \llbracket e_i \rrbracket_e, \ldots \llbracket e_m
            \rrbracket_e)\rrbracket$
            which is equal to 
            \[
\llbracket agg(\llbracket e_1 \rrbracket_e, \llbracket e_2 \rrbracket_e, \ldots,
            \llbracket m(\llbracket e_1 \rrbracket_e, \llbracket e_2 \rrbracket_e, \ldots,
            \llbracket e_i \rrbracket_e, \ldots \llbracket e_m
            \rrbracket_e)\rrbracket, \ldots \llbracket e_m
            \rrbracket_e)\rrbracket
            \]
            by definition of Parallelizable Pure commands.
    \end{itemize}
\end{proof}



\begin{theorem}
    \label{thm:equi_prog}
    For any given Dataflow transformation program $p$, if $p \Longrightarrow_t
    p'$ then $p \equiv p'$.
\end{theorem}
\begin{proof}
    \begin{itemize}
        \item {\bf Unused}: If $g$ is no side-effectful and variable $x_i$ is
            not used as a parameter in any other function or in the return
            statement, we can remove this assignment without affecting any
            symbolic expressions in the return statement. 
        \item {\bf Commute}: If both $g_1$ and $g_2$ are not simulatenously
            side-effectful, their effect on the system will not confict. Since
            $g_2$ does not use $x_i$, we can switch the order of assignments to
            $x_i$ and $x_j$ without affecting any other expressions which uses
            $x_i$ and $x_j$.
        \item {\bf Var-Change}: Since we change any references of $x_i$ is the
            rest of the program to $x_j$, and $x_j$ is not being assigned again
            (we do not break the constraint that each variable is only assigned
            once), we can change the variable name without affecting the
            symbolic expressions constructed.
        \item $\relay$ acts as an identity, therefore symbolic expression for 
            $x_i$ and $x_j$ are equivalent. Any expression constructed using
            them are equivalent before the transformation. 
        \item Using Theorem~\ref{thm:equi_exp}, for {\bf concat-split,
            split-concat, multi-concat, multi-split} 
            the symbolic expression for
            $x_i$ and $x_j$ are equivalent. Any expression constructed using
            them are equivalent to the version before the transformation.
        \item Using Theorem~\ref{thm:equi_exp}, for {\bf stateless} and {\bf
            parallelizable Pure} transformations, the expression of $x_k$ is
            equivalent to the one before the transformation. Any expression
            constructed using $x_k$ is equivalent to version before the
            transformation.
    \end{itemize}
\end{proof}


==> revision-cover.tex <==


We have addressed all mandatory revision changes that the reviewers asked for.
We haven't yet addressed all the rest of the review comments (such as typos and presentation improvement suggestions), but we will address them in the final version of the paper.

To aid reviewers, we have marked all the changes with a dark blue color so that they are easier to distinguish from the rest of the text.
We also provide a list of the required changes and how we addressed them here.

\begin{enumerate}
    \item \textit{Explain the role of PaSh annotations and how they relate (as
    axioms) to soundness:} This is addressed partly in \sx{shell2dfg} (Shell Scripts
    to DFGs) and partly in \sx{related} (Related Work, par. ``Parallel Shell
    Scripting''), where PaSh and POSH are discussed.
    \item \textit{Discuss giving users direct access to the IR:}
    This is addressed partly in \sx{eval} (Evaluation, par. ``Implementation'') and partly \sx{discussion} (Discussion, par. ``Directly accessing the IR in the implementation'').
    \item \textit{Discuss how you've debugged scripts, with `relay' or otherwise:}
    This is addressed in \sx{discussion} (Discussion, par ``Parallel Script Debugging'').
    \item \textit{Motivate the ``large but finite'' problem domain --- as opposed to
    infinite streams:}
    This is addressed partly at the end of \sx{model:prelim} (Preliminaries) and in \sx{discussion} (Discussion, par. ``Stream Finiteness and Extensions'').
    \item \textit{Briefly relate the ODFG model to the PaSh and POSH IRs:}
    This is addressed mostly in \sx{related} (Related Work, par. ``Parallel Shell Scripting''), where PaSh and POSH are discussed.
    \item \textit{Say that POSH uses different annotations and has slightly different goals:}
    This is addressed mostly in \sx{related} (Related Work, par. ``Parallel Shell Scripting''), where PaSh and POSH are discussed.
    \item \textit{Mention future work: infinite streams, more optimizations, more unix commands:}
    This is addressed at various points of \sx{discussion} (Discussion).
\end{enumerate}

\noindent
\textit{The revision need not:}
\begin{itemize}
    \item \textit{use Dash as a baseline --- we agree that Bash is fine}
    \item \textit{compare performance to POSH or PaSh --- a brief discussion of why
not is enough:}
    This is addressed mostly in \sx{related} (Related Work, par. ``Parallel Shell Scripting''), where PaSh and POSH are discussed.
\end{itemize}


